Oracle Efficient Private Non-Convex Optimization

One of the most effective algorithms for differentially private learning and optimization is objective perturbation. This technique augments a given optimization problem (e.g. deriving from an ERM problem) with a random linear term, and then exactly solves it. However, to date, analyses of this approach crucially rely on the convexity and smoothness of the objective function, limiting its generality. We give two algorithms that extend this approach substantially. The first algorithm requires nothing except boundedness of the loss function, and operates over a discrete domain. Its privacy and accuracy guarantees hold even without assuming convexity. This gives an oracle-efficient optimization algorithm over arbitrary discrete domains that is comparable in its generality to the exponential mechanism. The second algorithm operates over a continuous domain and requires only that the loss function be bounded and Lipschitz in its continuous parameter. Its privacy analysis does not require convexity. Its accuracy analysis does require convexity, but does not require second order conditions like smoothness. Even without convexity, this algorithm can be generically used as an oracle-efficient optimization algorithm, with accuracy evaluated empirically. We complement our theoretical results with an empirical evaluation of the non-convex case, in which we use an integer program solver as our optimization oracle. We find that for the problem of learning linear classifiers, directly optimizing for 0/1 loss using our approach can out-perform the more standard approach of privately optimizing a convex-surrogate loss function on the Adult dataset.

==> docs/objective.tex <==
\section{Objective perturbation over a discrete decision space}
\label{sec:discrete}
In this section we give an objective perturbation algorithm that is
$(\eps, \delta)$-differentially private for any non-convex Lipschitz
objective over a discrete decision space $\discspace$. We assume that
each $l\in \mathcal{L}$ is $G$-Lipschitz over $\discspace$
w.r.t. $\ell_2$ norm: that is for any $w, w'\in \discspace$,
$|l(w) - l(w')| \leq G \|w - w'\|_2$. Note that if $l$ takes values in
$[0, 1]$, then we know $l$ is also $1/\tau$-Lipschitz due to the
$\tau$-separation in $\discspace$.


\paragraph{The Normalization Trick}. The key technical innovation in this section of the paper is the modification of the standard objective perturbation algorithm by introducing a normalization step: rather than minimizing the perturbed loss, we minimize the perturbed normalized loss. Let $D$ be a bound on the maximum $\ell_2$ norm of any vector in
$\discspace$. We will make use of a normalization onto the unit sphere in one higher dimension. The normalization function $\bprojI:\mathbb{R}^d\rightarrow \mathbb{R}^{d+1}$ is defined as:
$$\bproj{w} = \left(w_1, \ldots, w_d, D\sqrt{1-\|w\|_2^2/D^2}\right) \frac{1}{D}$$
%
Note that $\|\bproj{w}\|_2 = 1$ for all $w\in\discspace$,  and also that for any $w,w' \in\discspace$,
\begin{equation}
\label{projfact}
\| \bproj{w} -\bproj{w'}\|_2^2  \geq \frac{1}{D^2} \|w-w'\|_2^2,
\end{equation}
since $\| \bproj{w} -\bproj{w'}\|_2^2 = \frac{1}{D^2}(\|w-w'\|_2^2 +  D^2(\sqrt{1-\|w\|_2^2/D^2}-\sqrt{1-\|w'\|_2^2/D^2})^2) \geq \frac{1}{D^2} \|w-w'\|_2^2$. This shows that normalizing into the $(d+1)$-dimensional sphere  can't force points too much closer together than they start. The intuition behind the privacy proof is that the linear perturbation term provides stability; specifically we will argue that for any value of the noise $\eta$ than induces a particular minimizer $\hat{w}$ on a dataset $\DS$, there is a nearby value $\eta'$ that would induce $\hat{w}$ on any adjacent dataset $\DS'$. The argument proceeds by contradiction: suppose that there existed some $v \neq \hat{w}$ that was the minimizer on $\DS'$. Then since $\DS$ and $\DS'$ only differ in one data point, the difference between the normalized losses of $v$ and $\hat{w}$ on $\DS'$ can be broken into three terms: the difference between their scores on $\DS$ and the original perturbation term $\eta$, the difference between their scores on the two data points that differ between $\DS, \DS'$,
%
% The first term is positive by virtue of $\hat{w}$ being the minimizer on the original dataset $\DS$. The second term can be lower bounded using Lipschitzness of $\mathcal{L}$. The third term is lower bounded using the fact that $\eta'-\eta$ is chosen to maximize the inner product with $\hat{w}$ by making the change in noise $\eta'-\eta$ move in the direction of $\pi(\hat x)$
% We can only guarantee this has a greater inner product with $\hat{w}$ than $v$ if $||\hat{w}|| = ||v||$, which is the rationale behind the normalization trick. Then the whole expression can be shown to be lower bounded by $0$, contradicting the fact that $v$ is the unique minimizer of the normalized loss on $\DS'$.
% }
% \sout{and the difference between their inner product with $\eta'-\eta$.}
and the inner product between their normalized difference $\pi(\hat w)-\pi(v)$
with $\eta' - \eta$.
 The first term is positive by virtue of $\hat{w}$ being the minimizer on the original dataset $\DS$. The second term can be lower bounded using Lipschitzness of $\mathcal{L}$.
The third term is lower bounded using the fact that $\eta'-\eta$ is chosen to maximize the inner product $\inner{\eta'-\eta }{\pi(\hat w) - \pi(v)}$ by making the change in noise $\eta'-\eta$ move in the direction of $\pi(\hat w)$
% \sout{We can only guarantee this has a greater inner product with $\hat{w}$ than $v$ if $||\hat{w}|| = ||v||$}
We can only guarantee this has a greater inner product with $\hat{w}$ than $v$ if $\|\pi(\hat{w})\|_2 = \|\pi(v)\|_2$
, which is the rationale behind the normalization trick. Then the whole expression can be shown to be lower bounded by $0$, contradicting the fact that $v$ is the unique minimizer of the normalized loss on $\DS'$.


%% Algorithm: Objective Perturbation
\begin{algorithm}[H]
\label{algorithm:objper}
\SetAlgoLined
\KwIn{$\dataset = \{ l_i \}_{i=1}^n$, oracle $\oracle_{\pi}$ over $\discspace$, privacy parameters $\epsilon$, $\delta$}
$\sigma \leftarrow  \frac{7 G D^2 \sqrt{\ln{1/\delta}}}{\tau \epsilon}$ \;
Draw random vector $\eta \sim \mathcal{N} \big(0, \sigma^2 \big)^{d+1}$ and use the projected oracle to solve:
% $$w \in \argmin_{w \in \discspace}\bigg( \lossregnormedValue{\dataset}{w}{\eta} \bigg)$$
\[
  \hat w = \oracle_{\pi}(\DS, \eta) \in \argmin_{w\in \discspace}\lossregnormed_\pi(\DS, \eta, w)
\]
%

\KwOut{$\hat w$}
\caption{Objective Perturbation over Discrete Space \ObjDisc}
\end{algorithm}
%
%
%
%

%%%%%%%%%%%%%%%
%% Privacy
%%%%%%%%%%%%%%%
\paragraph{Privacy Analysis}
We now  prove that $\ObjDisc$ is differentially private, illustrating the importance of the normalization trick. We then state an accuracy bound, which follows from a simple tail bound on the random linear perturbation term.
% \subsection{Privacy}
We defer the full proof  to the Appendix.
\begin{theorem}\label{dproof}
Algorithm \ref{algorithm:objper} is $(\epsilon, \delta)$-differentially private.
\end{theorem}

\begin{proof}[Proof Sketch]
For any realized noise vector $\eta$, we write $\wopt = \oracle_\pi(\DS, \eta)$ as the output. We first want to show that there exists a mapping $\noisemap{\wopt}:\mathbb{R}^{d+1}\rightarrow\mathbb{R}^{d+1}$ such that $\wopt$ is the parameter vector output on any neighboring dataset $\DS'$ when the noise vector is realized as $\noisemap{\wopt}(\eta)$: that is, $\wopt = \oracle_\pi(\DS',\noisemap{\wopt}(\eta))$. If we can show that $\pr{\eta} \approx \pr{\noisemap{\wopt}(\eta)}$, then the probability of outputting any particular $w$ on input $\DS$ should be close to the corresponding probability, on input $\DS'$ as desired.

 Denote  the set of of noise vectors that induce output $w$ on dataset $\DS$ by $\noiseset{\DS, w} =\{\eta : \oracle_\pi(\DS, \eta)=w  \}$.
Define our mapping:
$$\noisemap{\wopt}(\eta) = \eta + \frac{2}{\tau } G D^2 \bproj{\wopt}  $$
%%
%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%
%% Lemma: indicator
%%%%%%%%%%%%%%%%%%%
We now state $3$ key lemmas. First, Lemma~\ref{lemma:indicator} shows that our mapping preserves the minimizer $\hat{w}$ even after switching to the adjacent dataset $D'$; so long as the minimizer is unique.
\begin{lemma}
\label{lemma:indicator}
Fix any $\wopt$ and any pair of neighboring datasets $\DS,\DS'$. Let $\eta \in \noiseset{\DS, \wopt}$ be such that $\wopt$ is the unique minimizer $\wopt \in \inf_w \loss(\DS, w)-\inner{\eta}{\bproj{w}}$. Then $\noisemap{\wopt}(\eta)\in \noiseset{\DS', \wopt}$. Hence:
%%
$$\mathbbm{1}\{ \eta \in \noiseset{\DS, \wopt}\} \leq \mathbbm{1}\{ \noisemap{\wopt}(\eta)\in \noiseset{\DS', \wopt}\}$$
\end{lemma}
%%
%%
\begin{proof}
Let $c=\frac{4}{\tau } G D^2$. Suppose that $\wcon \neq \hat{w}$ is the output on neighboring dataset $\DS'$ when the noise vector is $\noisemap{\wopt}(\eta)$. We will derive a contradiction. Since $v$ is the unique minimizer on $\DS'$:
%% 1st equation
\begin{equation}\begin{split}
\label{eq:dprimegap}
\Big(\lossF{\dataset', \wcon}-\inner{\noisemap{\wopt}(\eta)}{\bproj{\wcon}}\Big) - \Big(\lossF{\dataset', \wopt}-\inner{\noisemap{\wopt}(\eta)}{ \bproj{\wopt}} \Big)
<0
\end{split}\end{equation}
%% Space
Let $i$ be the index where $\DS$ and $\DS'$ are different, such that $l_i \in \DS$ and $l_i^{'} \in \DS'$. Then $\lossF{\DS', w} = \lossF{\DS, w} - l_i(w) + l_i^{'}(w)$. Now, write the loss function in terms of $\dataset$ and rearranging terms:
%% 2nd equation
\begin{equation*}
\begin{split}
\bigg[ \Big(\lossF{\dataset, \wcon}-\inner{\eta}{ \bproj{\wcon}}\Big) - \Big(\lossF{\dataset, \wopt}-\inner{\eta}{ \bproj{\wopt}} \Big)\bigg] + \big(l_i(\wopt)-l_i(\wcon)\big) - \big(l_i^{'}(\wopt)-l_i^{'}(\wcon)\big)\\
+\inner{c\bproj{\wopt}}{ \bproj{\wopt}} - \inner{c\bproj{\wopt}}{ \bproj{\wcon}} < 0
\end{split}
\end{equation*}
%
Since $\wopt$ is a unique minimizer for $\DS$ and $\eta$ then term in the square bracket is positive. Hence:
\begin{equation*}
\begin{split}
 \big(l_i(\wopt)-l_i(\wcon)\big) - \big(l_i^{'}(\wopt)-l_i^{'}(\wcon)\big) +\inner{c\bproj{\wopt}}{ \bproj{\wopt} - \bproj{\wcon}} < 0
\end{split}
\end{equation*}
%
Since $l_i, l_i'$  are $G$-Lipschitz functions $v\big(l_i(\wopt)-l_i(\wcon)\big) - \big(l_i^{'}(\wopt)-l_i^{'}(\wcon)\big) \geq -2G\|\wopt-\wcon\|_2$. Also, $\inner{c\bproj{\wopt}}{ \bproj{\wopt}-\bproj{\wcon}} = \frac{c}{2}\|\bproj{\wopt}-\bproj{\wcon}\|_2^2$, by expanding  $\|\bproj{\wopt}-\bproj{\wcon}\|_2^2$ and using $||\pi(v)||_2 = ||\pi(\hat{w})||_2 = 1$.
Substituting this becomes:
%% 4th equation
\begin{equation*}
\begin{split}
-2G\|\wopt-\wcon\|_2 +\frac{c}{2}\|\bproj{\wopt}-\bproj{\wcon}\|_2^2 < 0
\end{split}
\end{equation*}
Since $\|\bproj{\wopt}- \bproj{\wcon}\|_2^2 \geq \frac{1}{D^2}\|\hat{w}-v\|_2^2$: %% 5th equation
\begin{equation}\begin{split}
-2G\|\wopt-\wcon\|_2 +\frac{c}{2D^2} \|\wopt-\wcon\|_2^2 &< 0 \\
\frac{c}{2D^2}\|\wopt-\wcon\|_2 &< 2G \quad \text{Divide both sides by } \|\wopt-\wcon\|_2\\
c\|\wopt-\wcon\|_2 &< 4 G D^2 \\
c\tau &< 4 G D^2 \quad \text{By assumption }\wopt \neq \wcon,\text{ hence }\|\wopt-\wcon\|_2\geq \tau\\
c &< \frac{4 G D^2 }{\tau } \quad \text{Divide both sides by } \tau
\end{split}
\end{equation}
This contradicts $c = \frac{4 G D^2 }{\tau }$.
\end{proof}
%
%
Lemma~\ref{lemma:uniquew} shows that the minimizer is  unique with probability $1$.


\begin{lemma}% [\citep{neel2018use}]
\label{lemma:uniquew}
Fix any $\tau$-separated vector space $\discspace$. For every dataset $\DS$ there is a subset $B\subset \mathbb{R}^{d+1}$ such that $\pr{\eta \in B} = 0$ and for any $\eta \in \mathbb{R}^{d+1}\setminus B$:
$$ \exists \text{ a unique minimizer } \wopt \in \argmin_{w\in \discspace} \lossF{\DS,w}-\inner{\eta}{\bproj{w}}$$
\end{lemma}
%%

Finally Lemma~\ref{lem:gauss_ratio} shows that with high probability over the draw of $\eta$, $\pr{\eta} \approx \pr{\noisemap{\wopt}(\eta)}$.

\begin{lemma}
\label{lem:gauss_ratio}
Let $\eta \sim \mathcal{N}(0, \sigma^2)^{d+1}, \sigma \gets \frac{7G^2D^2\sqrt{\log(1/\delta}}{\tau \epsilon}, w \in \mathcal{W}_\tau$. Then there exists a set $C \subset \mathbb{R}^{d+1}$ such that $\pr{\eta \in C^{c}} \geq 1-\delta$, and for all $r \in C^{c}$ if $p$ denotes the probability density function of $\eta$:
$$
\frac{\pdf(r)}{\pdf(\noisemap{w}(r))} \leq e^{\epsilon}
$$
\end{lemma}
Finally, we focus on noise vectors $\eta$ in the set of
$A = \mathbb{R}^{d+1} \setminus (C \cup B)$, which has probability
mass at least $1 - \delta$, and show that for any $\eta$ in $A$ that
induces output solution $\hat w$ on $\DS$, the noise vector
$g_{\hat w}(\eta)$ also induces $\hat w$ on the neighbor $\DS'$. Then
the $(\epsilon,\delta)$-differential privacy guarantee essentially
follows from the bounded ratio result in Lemma~\ref{lem:gauss_ratio}.
%%
%
%
\end{proof} %% proof of (eps,delta)-DP theorem
%
%



%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%
%% Theorem: accuracy
%%%%%%%%%%%%%%%%%%%

We now state the accuracy guarantee, which follows from a standard Gaussian tail bound. Then in Subsection~\ref{sec:compare} we compare this guarantee to the accuracy guarantee for the competing RSPM method for learning discrete hyperplanes, in order to shed some light on the accuracy guarantee in practice.
\begin{theorem}[Utility]\label{theorem:objperUtility}
Algorithm \ref{algorithm:objper} is an ($\alpha,\beta$)-minimizer for $\discspace^*$ with
%% Space
$$\alpha = \frac{2\sqrt{2(d+1)\ln{(4/\beta)}}\sigma}{n} = \frac{14 G D^2\sqrt{2(d+1)\ln{(4/\beta)}\ln{(1/\delta)}}}{n\tau \epsilon}$$
\end{theorem}
\begin{proof}

For $S \sim \mathcal{N}(0, \sigma^2)$ we have the following tail bound:
%% 1st equation
$$\pr{S \geq t} \leq 2 \exp{\Big(-\frac{t^2}{2\sigma^2} \Big)}$$
%

Now let $S = \sum_{i=1}^{d+1} \eta_i$ where each $\eta_i$ is a Gaussian random variable with variance $\sigma^2$. It follows that $S \sim \mathcal{N}(0, \sigma_S^2)$ for $\sigma_S^2 = (d+1)\sigma^2$. With probability $1-\beta/2$ we have:
%% 2nd equation
$$\sum_{i=1}^{d+1} \eta_i \leq \sqrt{2(d+1)\ln{(2/\beta)}}\sigma = C$$
%% Space
Thus with probability $1-\beta/2$,
$$\sup_{w \in W_{\tau}}\inner{\eta}{\bproj{w}} \leq \sup_{\eta/C \in \Delta^{d+1}, ||y||_2 = 1}\inner{y}{\eta} = \sup_{||y||_2 = 1}  C||y||_{\infty} \leq C = \sqrt{2(d+1)\ln{(2/\beta)}}\sigma$$
%% Space
By symmetry with probability $1-\beta/2, \sup_{w \in W_{\tau}}\inner{\eta}{\bproj{w}} \geq -\sqrt{2(d+1)\ln{(2/\beta)}}\sigma$. Thus by a union bound, with probability $1-\beta, \sup_{w \in W_{\tau}}|\inner{\eta}{\bproj{w}}| \leq \sqrt{2(d+1)\ln{(2/\beta)}}\sigma$.

Let $w$ be the output of algorithm \ref{algorithm:objper} and $\wopt$ be the minimizer for $\DS$. Then  with probability $1-\beta$: $\lossregnormed_\pi(\DS,w,\eta) \geq \frac{\lossF{\DS, w} - \sqrt{2(d+1)\ln{(4/\beta)}}\sigma}{n}$
and
$ \lossregnormed_\pi(\DS,\wopt,\eta) \leq \frac{\lossF{\DS, \wopt} + \sqrt{2(d+1)\ln{(4/\beta)}}\sigma}{n} $.
%% Space
Combining these two bounds we get:
%% 4th equation
\begin{equation}
\begin{split}
\frac{1}{n}\lossF{\DS, w} \leq \lossregnormed_\pi(\DS,w,\eta) + \frac{\sqrt{2(d+1)\ln{(4/\beta)}}\sigma}{n} \\
\leq \lossregnormed_\pi(\DS,\wopt,\eta) + \frac{\sqrt{2(d+1)\ln{(4/\beta)}}\sigma}{n} \\
\leq \frac{\loss(\DS,\wopt)}{n} + 2\frac{\sqrt{2(d+1)\ln{(4/\beta)}}\sigma}{n}
\end{split}
\end{equation}

The second inequality is because $w$ is the minimizer for the regularized loss $\lossregnormed_\pi$
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Comparing
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Comparing $\ObjDisc$ and RSPM}
\label{sec:compare}
While both \ObjDisc{} and the RSPM algorithm of \cite{neel2018use}
require discrete parameter spaces, $\ObjDisc$ is substantially more
general in that it only requires the loss functions be Lipschitz,
whereas RSPM assumes the loss functions are bounded in $\{0, 1\}$ (and
hence $1/\tau$ Lipschitz over $\discspace$) and assumes the existence
of a small separator set (defined in the appendix). Nevertheless, we
might hope that in addition to greater generality, $\ObjDisc$ has
comparable or superior accuracy for natural classes of learning
problems. We show this is indeed the case for the fundamental task of
privately learning discrete hyperplanes, where it is better by a
linear factor in the dimension. We define the RSPM algorithm, for
which we must define the notion of a separator set, in the appendix.


\begin{theorem}[RSPM Utility \cite{neel2018use}]
\label{theorem:rspmUtility}
Let $\discspace^*$ be a discrete parameter space with a separator set of size $m$. The Gaussian RSPM algorithm is an oracle-efficient $(\alpha, \beta)$-minimizer for $\discspace^*$ for:
$$\alpha = O\bigg(\frac{m\sqrt{m \ln(2m/\beta) \ln(1/\delta)}}{\epsilon n}\bigg)$$
\end{theorem}
Let  $I_\tau$ be a $\tau$ discretization of $[-1, 1]^d$, e.g. $I_\tau = [-1, -1 + \tau, \ldots 0, \tau, 2\tau, \ldots 1]^{d}$. Let $W_\tau$ be the subset of vectors in this discretization that lie within the unit Euclidean ball: $W_\tau = I_\tau \cap S(1)^{d}$. $W_\tau$ is $\tau$-separated since any two distinct $w, w'$ differ in at least one coordinate by at least $\tau$. Moreover $W_\tau$ admits a separator set of size $m = \frac{2(d-1)}{\tau}$ (see the Appendix of \cite{neel2018use}. Since the loss functions $l_i(w) = \textbf{1}\{w \cdot x_i  \geq 1 \} \in \{0, 1 \}$ and $W_\tau$ is $\tau$-separated, the loss functions $l_i$ are $\frac{1}{\tau}$-Lipschitz.
By Theorem~\ref{theorem:rspmUtility}, RSPM has accuracy bound:
$$\alpha_{\text{RSPM}} = O\left(\frac{d \sqrt{d \log(d/\beta \tau)\log(1/\delta)}}{\tau \sqrt{\tau} \epsilon n}\right)$$
By Theorem~\ref{theorem:objperUtility} $\ObjDisc$ has accuracy bound:
$$
\alpha_{\ObjDisc} = O\left(\frac{\sqrt{d\log(1/\beta)\log(1/\delta)}}{n\tau^2 \epsilon}\right)
$$

Thus, in this case \ObjDisc{} has an accuracy bound that is better by
a factor of roughly $d\sqrt{\tau}$.




%%%%% Commented out
\iffalse
Let $\mathcal{W}$ denote the $\ell_2$-bounded continuous space of half space vectors. A database $\mathcal{X}\subset\mathbb{R}^d$ is a set of $d$-dimensional vectors representing the private data that we have access to. Let $n=|\mathcal{X}|$ be the number of records in $\mathcal{X}$. For the $i^{th}$ record $x_i\in\mathcal{X}$ and $w\in\mathcal{W}$ the $i^{th}$ $0 1$ loss function is:
%
\[
l_i(w)=
\begin{cases}
1 & \text{if } \inner{w}{x_i} >0\\
0 & \text{otherwise}
\end{cases}
\]
%
Since the private algorithms that we present in this paper are not suitable for learning continous spaces we must contruct a finite discretized approximation of $\mathcal{W}$ which we denote by $\discspace$. The set $\discspace$ is simple to construct, where each element $w$ in $\discspace$ can be writen as $w = \tau z $ where $z \in \mathbb{Z}^d$ and $\|w\|_2 < D$. Notice that under this regime the separator set size for $RSPM$ is $m=d/\tau$. In order to do a side by side comparison for algorithms \ref{algorithm:objper} and \ref{algorithm:rspm} let us rewrite the accuracy of RSPM from theorem \ref{theorem:rspmUtility} in terms of $d$ and $\tau$:

$$\alpha_{rspm} = O\bigg(\frac{d\sqrt{d \ln(2d/(\beta\tau)) \ln(1/\delta)}}{\epsilon\tau\sqrt{\tau} n}\bigg)$$


Furthermore, notice that the $01$ loss with domain $\discspace$ has lipschitz constant $G=1/\tau$. Therefore, replacing in the value of $G$ in theorem \ref{theorem:objperUtility} we get that Algorithm \ref{algorithm:objper} has accuracy:

$$\alpha_{op} = \frac{2\sqrt{2(d+1)\ln{(1/\beta)}}(3.5 D^2 \sqrt{\ln{1/\delta}})}{N\tau^2 \epsilon}$$


\fi
% $\mathcal{W}$

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "neurips_2019"
%%% End:


==> docs/privacy.tex <==
\section{Privacy Analysis of $\PUCB$}

We show that releasing the sequence of actions by
algorithm $\PUCB$ satisfies JDP with respect to any user on an episode
changing his data. Formally,
\begin{theorem}\label{thm:jdp}
Algorithm (\ref{alg:pucb}) \PUCB~is $\eps$-JDP.
\end{theorem}

To prove theorem \ref{thm:jdp}, we use the \emph{billboard lemma} due
to \cite{hsu2016private} which says that an algorithm is JDP if the
output sent to each user is a function of the user's private data and
a common signal computed with standard differential privacy.
We state the formal lemma:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Lemma billboard
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}[Billboard lemma \cite{hsu2016private}]\label{lem:billboard}
Suppose $\algo:U \rightarrow \cR$ is $\eps$-differentially
private. Consider any set of functions $f_i : U_i\times \cR \rightarrow \cR'$
where $U_i$ is the portion of the database containing the $i$'s user
data. The composition $\{f_i(\Pi_i U, \algo(U))\}$ is
$\eps$-joint differentially private, where $\Pi_i:U\rightarrow U_i$
is the projection to $i$'s data.
\end{lemma}

Let $U_{<t}$ denote the data of all users before episode $t$
and $u_t$ denote the data of the user during episode $t$.
Algorithm  \PUCB keeps track of all events on users $U_{<t}$
% using $SAH$ parallel
in a differentially-private way with private counters
$\rtilt, \ntilt, \mtilt$.
These counters are given to the procedure \PrivQ~ which computes a
$Q$-function
$\QtilUB_t$, and induces the policy $\pit(s,h) \coloneqq \max_a \QtilUB_t(s,a,h)$
to be use by the agent during episode $t$.
%
Then the output during episode $t$ is generated the policy $\pit$
and the private data of the user $u_t$ according to the protocol
\ref{alg:rlprotocol},
 the output on a single episode is:
 $\left(\pit\left(s^{(t)}_1, 1\right), \ldots,  \pit\left(s^{(t)}_H, H\right)\right)$.
%
By the billboard lemma \ref{lem:billboard}, the composition of the output
of all T episodes, and the final policy
$\left(\left\{\left( \pit(s^{(t)}_1, 1), \ldots,  \pit(s^{(t)}_H, H)\right) \right\}_{t\in [T]}, \pi_T\right) $
satisfies $\eps$-JDP if the policies
$\{\pit\}_{t\in [T]}$  are computed with a $\eps$-DP mechanism.

Then it only remains to show that the noisy counts satisfy $\eps$-DP.
%
First, consider the counters for the number of visited states.
 The algorithm $\PUCB$ runs $SAH$
parallel private counters, one for each state tuple $(s,a,h)$.
Each counter is instantiated with a $\eps/(3H)$-differentially
private mechanism which takes an input an event stream
$\nhat(s,a,h) = \{0,1\}^T$ where the $i$th bit is set to 1 if
a user visited the state tuple $(s,a,h)$ during episode $i$ and
0 otherwise. Hence each stream $\nhat(s,a,h)$ is the data
for a private counter. The next claim says that the total $\ell_1$
sensitivity over all streams is bounded by $H$:
%
\begin{claim}\label{claim:sensitivity}
Let $U, U'$ be two $t$-neighboring user sequences, in the sense that they
are only different in the data for episode $t$.
For each $(s,a,h)\in\states\times\actions\times [H]$,
let $\nhat(s,a,h)$ be the event stream corresponding to user sequence
U and $\nhat'(s,a,h)$  be the event stream corresponding to $U'$.
Then the total $\ell_1$ distance of all stream is given by the following
claim:
% The event stream has $\ell_1$ sensitivity equal to $H$.
\begin{align*}
  \sum_{(s,a,h)\in \states\times\actions\times [H]} \|\nhat(s,a,h)
  -\nhat'(s,a,h)\|_1\leq H
\end{align*}
\end{claim}
\begin{proof}
The proof follows from the fact that on any episode $t$
a user visits at most $H$ states.
\end{proof}

Finally we use a result from \citep[Lemma 34]{hsu2016private}
which states that the
composition of the $SAH$
$(\eps/3H)$-DP counters for $\nhat(\cdot)$ satisfy $(\eps/3)$-DP
as long as the $\ell_1$
sensitivity of the counters is $H$ as shown in
claim \ref{claim:sensitivity}.
We can apply the same analysis to show that the counters corresponding
to the empirical reward $\rhat(\cdot)$ and the transitions $\mhat(\cdot)$
are both also $\eps/3$-differentially private.
% %
Putting it all together releasing the noisy counters is $\eps$-differentially private.

